Coverings of open books

We study a coverings of open books and virtually overtwisted contact manifolds using open book foliations. We show that open book coverings produces interesting examples such as transverse knots with depth grater than 1. We also demonstrate explicit examples of virtually overtwisted open books.

==> labelfig.tex <==
 %%%%%%%%%%%%%%%%%%%--------------- CUT
 
  %%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%
 %%%%%   LabelFig.tex FOR LABELLING FIGURE INSERTS %%%%%
  %%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%
 %%%  AUTHOR: Laurent Siebenmann
  %%    lcs@matups.matups.fr
  %%
 %%%  VERSION: July 1991
  %%
 %%%  PURPOSE:
  %%  Occasionally, figures imported into TeX lack some labels.
  %%  It may then be most convenient to use TeX to provide
  %%  the labels.  Several macro sets, notably the
  %%  LaTeX picture environment, provide means to insert
  %%  labels.  LabelFig.tex is a small (4Ko) and fast macro file
  %%  offering labelling capability for other TeX formats such
  %%  as Plain and AmSTeX.  Hopefully it will work in essentially
  %%  all TeX environments.
  %%
 %%%  THE IDEA:
  %%  Nothing distinctly new here.
  %%  Each label is located with respect
  %%  to a grid laid down on the figure --- as in LaTeX.
  %%  The device of using TeX to print the grid in proof versions
  %%  is apparently not in LaTeX but has been since used by
  %%  others.  Many thanks to to Raymond Seroul (Strassbourg) for
  %%  pointing it out to me back in 1989.
  %%  (It was used in a Plain TeX hack of the picture
  %%  environment by Desarmenien, Ostromoukhov, and Seroule
  %%  that seems not to have been released.)
  %%
 %%%  POSTINGS (soon!!): anonymous ftp
  %%  ---  ftp 28.146.7.200 (alias shape.mps.ohio-state.edu);
  %%  login: anonymous;  password: <anything>;
  %%  directory pub/osutex
  %%  ---  ftp 130.84.128.100 (alias rsovax.circe.fr);
  %%  login: anonymous; password: <anything>; directory
  %%  [anonymous.siebenmann]
  %%
 %%%% DOCUMENTATION:
  %%  --- see Labelfig.doc
  %% (may be included at end, after \endinput)
  %%
 %%%% EXAMPLE OF USAGE:
  %%    \input LabelFig.tex
  %%    \SetLabels
  %%      (.3*.7) first label\\
  %%         % label will go to position .3 from left
  %%         % and .7 from bottom
  %%      \L(.61*.333) $\Lambda_1\leq\Gamma$\\
  %%         % \L places left edge of label
  %%         % (rather than the center)
  %%         % similarly use \R for right edge;
  %%         % and \B for bottom or \T for top
  %%      \T\R(.3*.7) last label \\
  %%    \endSetLabels
  %%    \ShowGrid
  %%         % lays grid on figure to label;
  %%         % delete for final printing
  %%    \AffixLabels{\BoxedEPSF{MyFigure}}
  %%         % argument of \AffixLabels#1 should be a TeX box
  %%         % covering the inserted figure to be labelled.
  %%         % (Here \BoxedEPSF is the figure insertion macro
  %%         % of my package \BoxedEPS.tex (same sources)
  %%         % for inserting encapsulated PostScript graphics.
  %%         % But any other means of inserting
  %%         % the figure can be used.)
 
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 %%%%% FORBID REREADING %%%%%
  %
  \ifx \LabelFigloaded\MYundefined
  \else
    \immediate\write16{ !!! LabelFig.tex ALREADY loaded.}
  \endinput\fi
 
  \def\LabelFigloaded{\relax}% now loaded
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%% Beyond this point we use some control sequences
  %%% that are 'padlocked'  with @ of category 11
 
  \chardef\LabelFigCatAt\the\catcode`\@
  \catcode`\@=11
 
 %%temporarily suppress Plain's logging of allocations
 \let\LabelFigwlog@ld\wlog
 \def\wlog#1{\relax}
 
 
 \ifx\\\MYundefined@
    \let\\\relax
 \fi
 
 \def\N@wif{\csname newif\endcsname }
 \def\Temp@ {\N@wif\ifIN@}
 \ifx\INN@\MYundefined@
    \else \let\Temp@\relax
 \fi
 \Temp@
 
  %%% \IN@0#1@#2@ : Is 1st exp of #1 in 1st exp of #2 ??
   %% Answer in \ifIN@
  %\newif\ifIN@
  \def\IN@{\expandafter\INN@\expandafter}
  \long\def\INN@0#1@#2@{\long\def\NI@##1#1##2##3\ENDNI@
    {\ifx\m@rker##2\IN@false\else\IN@true\fi}%
     \expandafter\NI@#2@@#1\m@rker\ENDNI@}
  \def\m@rker{\m@@rker}
 
   %%% \Shifted@@#1#2#3 puts #3 in \hbox
   %% leaves basepoint as is
   %% then translates ink only by dims #1,#2
   %% with Postscript convention
   %% For simplicity use only on scrunched boxes
 \def\Shifted@@#1#2#3{\setbox0=\hbox{#3}%
   \raise -\dp0\vbox {\kern-#2%
       \hbox {\kern#1\box0\kern-#1}%
           \kern#2}}
 
 
 
 \newcount\gridcount
 \newbox\auxGridbox@ \newbox\hGridbox@ \newbox\vGridbox@
 \newbox\Labelbox@ \newbox\auxLabelbox@
 \newbox\Coordinatebox@
 \newtoks\Labeltoks@
 \newdimen\Wdd@ \newdimen\Htt@
 
 \def\hRule@{\advance\gridcount -2%
   \vskip-.2pt\hrule\vskip-.2pt\vfil
   \llap{\smash{\raise -2.5pt
     \hbox{.\number\gridcount\kern2pt}}}%
           \vskip-.2pt\hrule\vskip-.2pt\vfil}
 
 \def\vRule@{\advance\gridcount 2%
   \hskip-.2pt\vrule\hskip-.2pt\hfil
   \setbox\auxGridbox@=\vbox to 0pt
      {\vskip \Htt@\vskip 2pt
        \hbox{\kern-3.5pt.\number\gridcount}\vss}%
      \wd\auxGridbox@=0pt \box\auxGridbox@
   \hskip-.2pt\vrule\hskip-.2pt\hfil}
 
 \def\PlaceGrid@@{\gridcount=10%
  \setbox\hGridbox@=%
    \hbox{\hbox{\GridSpider@{\hskip-.4pt\vrule}%
             \vbox to \Htt@{\offinterlineskip\parindent=\z@%
                \GridSpider@{\vskip-.4pt\hrule}\vfil
                \hRule@\hRule@\hRule@\hRule@
                  \vskip-.2pt\hrule\vskip-.2pt\vfil
                \hbox to \Wdd@{\hfil}%
             \GridSpider@{\hrule\vskip-.4pt}}%
         \GridSpider@{\vrule\hskip-.4pt}}}%
  \gridcount=0%
  \setbox\vGridbox@=
     \hbox{\vbox{\offinterlineskip\parindent=0pt\hsize=0pt
       \GridSpider@{\vskip-.4pt\hrule}%
             \hbox to \Wdd@{%
                \GridSpider@{\hskip-.4pt\vrule}\hfil
                \vtop to \Htt@{\vfil}%
                     \vRule@\vRule@\vRule@\vRule@
                     \hskip-.2pt\vrule\hskip-.2pt\hfil
             \GridSpider@{\vrule\hskip-.4pt}}%
         \GridSpider@{\hrule\vskip-.4pt}}}%
  %
  \wd\hGridbox@=0pt\ht\hGridbox@=0pt
  \wd\vGridbox@=0pt\ht\vGridbox@=0pt
  %
 \hbox{\box\hGridbox@\box\vGridbox@}%
  }
 
 \def\SetLabels#1\endSetLabels{%
   \Labeltoks@={#1}}
 
 \def\GridSpider@#1{#1}
 \let\PlaceGrid@\relax
 \def\ShowGrid{\let\PlaceGrid@\PlaceGrid@@}
 
 \def\bAdjust@@{%
     \setbox\auxLabelbox@=\hbox{\raise \dp\auxLabelbox@
            \box\auxLabelbox@}}
 \def\bAdjust@{\let\vAdjust@\bAdjust@@}
 
 \def\tAdjust@@{%
     \setbox\auxLabelbox@=\hbox{\raise-\ht\auxLabelbox@
            \box\auxLabelbox@}}
 \def\tAdjust@{\let\vAdjust@\tAdjust@@}
 
 \let\vAdjust@\relax
 
 \def\lAdjust@{\let\hAdjust@\rlap}
 \def\rAdjust@{\let\hAdjust@\llap}
 
 \let\hAdjust@\relax\let\vAdjust@\relax
 
 \def\FetchLabel@#1(#2*#3)#4\\#5\endFetchLabel@{%
     %\globaldefs=1\setbox0=\hbox{#1}\globaldefs=0%
     \ignorespaces#1\unskip
     \Labeltoks@={#5}%
     \setbox\auxLabelbox@=%
        \hbox to 0pt{\hss\ignorespaces\hAdjust@
          {\ignorespaces#4\unskip}\hss}%
     \vAdjust@
     \let\hAdjust@\relax\let\vAdjust@\relax
     \setbox\Labelbox@=\hbox to 0pt{%
       \box\Labelbox@
       \Shifted@@{#2\Wdd@}{#3\Htt@}{\box\auxLabelbox@}}%
     \ht\Labelbox@=0pt\dp\Labelbox@=0pt
     }
 
 \def\PlaceLabels@@{\bgroup\def\Cr@{\\}%
     \let\L\lAdjust@\let\R\rAdjust@
     \let\B\bAdjust@\let\T\tAdjust@
     \loop
     \IN@0\Cr@ @\the\Labeltoks@ @\relax
     \ifIN@ \expandafter
       \FetchLabel@\the\Labeltoks@\endFetchLabel@
     \repeat
     \box\Labelbox@\egroup}%
 
 \let \PlaceLabels@\PlaceLabels@@
 
 \def\AffixLabels#1{\setbox\Coordinatebox@=\hbox{#1}%
      \Wdd@=\wd\Coordinatebox@ \Htt@=\ht\Coordinatebox@
      \advance\Htt@ \dp \Coordinatebox@
      \hbox{\copy\Coordinatebox@\kern-\Wdd@%
           \Shifted@@{0pt}{-\dp\Coordinatebox@}%
            {\PlaceGrid@\PlaceLabels@}%
           \kern\Wdd@}}
 
 %%% Restoring
   \let\wlog\LabelFigwlog@ld %%restore logging
   \catcode`\@=\LabelFigCatAt  %%12 or 13
 
  \endinput
 
 %% end of  LabelFig.tex

